Lagrangian Topology and Enumerative Geometry

We use the "pearl" machinery in our previous work to study certain enumerative invariants associated to monotone Lagrangian submanifolds.

==> Jones-map.tex <==
\subsection{Free loop representations of moduli spaces and the Jones map}
 Let $L$ be a closed, smooth manifold. We denote
by $\Lambda L$ the free loop space of $L$, $\Lambda L=L^{S^{1}}$.
There exists a map constructed by J.D.S. Jones \cite{Jo}
which establishes an isomorphism:
$$J: H_{k}(\Lambda L;\k)\to HH^{\ast,n-k}(C^{\ast}(L;\k),C^{\ast}(L;\k))$$
here $C^{\ast}(L;\k)$ is the co-chain algebra of $L$.
In this subsection we recall a few useful facts about this map.

\

We identify the $k$-simplex $\Delta^{k}$ with the $k$-tuples of points
$x_{1},\ldots, x_{k}\in\R$ with the property that $0\leq x_{1}\leq x_{2}\leq \ldots \leq x_{k}\leq 1$.
There is an evaluation map $\phi_{k}:\Delta^{k}\times \Lambda L\to L^{k+1}$ defined by
$\phi_{k}((x_{1},\ldots, x_{k}),\gamma)=(\gamma(0),\gamma(x_{1}),\ldots, \gamma(x_{k}))$.
To this map we can associate a chain morphism: $\tilde{\phi}_{k}:C_{s}(\Lambda L)\to
C_{s+k}(L^{k+1})$ (where $C_{\ast}( - )$ denotes the singular complex) as follows.
First for a simplex $\delta\in C_{s}(\Lambda L)$
we consider the composition
$$
\bar{\phi}_{k}(\delta)=\Delta^{k}\times\Delta^{s}\\
\stackrel{id\times\delta}{\longrightarrow} \Delta^{k}\times\Lambda L\stackrel{\phi_{k}}{\longrightarrow} L^{k+1}
$$  and we define $\tilde{\phi}_{k}$ as the sum of the composition of $\bar{\phi}_{k}(\delta)$  with
the $(k+s)$-simplices in a simplicial division of $\Delta^{k}\times \Delta^{s}$ (as the one used in defining the
singular cross-product).
We now write
$$C_{s+k}(L^{k+1})=\hom(C^{s+k}(L^{k+1}),K) = \hom^{-s-k}(C^{\ast}(L)^{\otimes_{k+1}},K)
=\hom^{-s-k}(C^{\ast}(L)^{\otimes _{k}}, C^{op}_{\ast}(L))$$
(where, for the second equality above we need $K$ to be a field; $V_{\ast}^{op}$ is the graded vector
space $V_{\ast}$ with the degrees reversed, the degree of $x\in V_{\ast}^{op}$ is $-deg_{V_{\ast}}(x)$).
Further:
$$\hom^{-s-k}(C^{\ast}(L)^{\otimes _{k}}, C^{op}_{\ast}(L))=\hom^{-s}((s^{-1}C^{\ast}(L))^{\otimes_{k}}, C^{op}_{\ast}(X))$$
and given that Poincar\'e duality gives an isomorphism: $C^{op}_{\ast}(L)\to C^{n+\ast}(L)$
we deduce an isomorphism: $\hom^{-s}((s^{-1}C^{\ast}(L))^{\otimes_{k}}, C^{op}_{\ast}(L))\to
\hom^{n-s}((s^{-1}C^{\ast}(L))^{\otimes_{k}}, C^{\ast}(L)) $.
We now denote by $\psi_{k}: C_{s+k}(L^{k+1})\to
\hom^{n-s}((s^{-1}C^{\ast}(L))^{\otimes_{k}}, C^{\ast}(L))$ the resulting isomorphism
and finally we put:
$$\tilde{J}: C_{s}(\Lambda L; \k)\to C^{\ast, n-s}(C^{\ast}(L),C^{\ast}(L)) \ , \ \tilde{J}=\psi_{k}\circ \tilde{\phi}_{k}~.~$$

It is shown by Jones that this map is a morphism of chain complexes  and that (under certain restrictions) it induces
an isomorphism in homology.

\begin{rem} \label{rem:grading - Hochshild} In the literature various other conventions
are used for the grading of the objects that appear in the Jones morphism. In particular,
if we grade the co-chain complex on $L$ as the graded $\hom$, $C^{\ast}(-)=\hom(C_{\ast}(-),K)$,
(thus with this convention co-homology is concentrated in negative degrees)
and if, simultaneously, in the definition of  Hochschild co-homology we use $s A^{\ast}$
 in the place of the de-suspension of $A^{\ast}$  (so that the Hochschild
 differential  becomes of bi-degree $(+1,-1)$), then  $J$ becomes a morphism of degree $-n$ with respect to
the second grading in Hochschild homology.
Geometrically, choosing this grading  of the co-chain complex is not natural and thus we have
not used these conventions here.
\end{rem}

There exists a spectral sequence with $E^{2}$ term $HH^{\ast}(H^{\ast}(L),H^{\ast}(L)$
which, under favourable conditions, converges to $HH^{\ast}(C^{\ast}(L),C^{\ast}(L)$.
In the case of the torus $T^{n}$ this spectral sequence actually collapses at the $E^{2}$ term
and we have a bigraded isomorphism $$HH^{\ast}(H^{\ast}(T^{n}),H^{\ast}(T^{n})\approx HH^{\ast}(C^{\ast}(T^{n}),C^{\ast}(T^{n})~.~$$

We are now interested in the part of the Jones chain map which lands in $C^{2,\ast}$.
By the description before this is is identified with the map
$\bar{\phi}_{2}$ which takes an $s$ simplex $\delta\in C_{s}(\Lambda L)$ and associates
to it the map
$$\bar{\phi}_{2}(\delta)((t_{1},t_{2}), (r_{1},\ldots r_{s}))=(\delta(r_{1},\ldots, r_{s})(0),
\delta(r_{1},\ldots, r_{s})(t_{1}), \delta(r_{1},\ldots, r_{s})(t_{2}))~.~$$
In other words this is simply the evaluation of the loops in the family $\delta$ in three
points the first being the origin. But this means that, in view of the definition of
the quantum product,  if we apply the Jones
map to a singular $n$-cycle representing the moduli space of $J$-homolorphic disks
of Maslov class $2$ and we project on to $HH^{2,\ast}$, then the resulting map
is precisely the infinitesimal $m_{1}$.


==> frobenius.tex <==
\section{Proof of Theorem~\ref{t:qh-frob-struct}} \label{prf:frob}

\INS





==> toric-old.tex <==
\section{Lagrangian tori in Toric manifolds} \label{s:toric} Here we work
out in detail the theory discussed in the previous sections for the
special case of Lagrangian tori that arise as fibres of the moment map
in a toric manifold. Below we will use in an essential way previous
results of Cho, Oh and of Fukaya-Oh-Ohta-Ono on Floer theory of torus
fibres in toric manifolds (see e.g.~\cite{Cho:Clifford,
  Cho-Oh:Floer-toric, Cho:products, FO3:toric-1, FO3:toric-2}). The
reader is refered to these papers for more details. For the
foundations of symplectic toric manifolds
see~\cite{Audin:torus-actions}, and for an algebro-geometric account
see~\cite{Fulton:toric-book}.

\subsection{Setting} \label{sb:toric-setting} Let $(M^{2n}, \omega)$
be a closed monotone toric manifold. Denote by $$\mathfrak{m}:M
\longrightarrow \textnormal{Lie}(\mathbb{T}^n)^* = \mathbb{R}^n$$ the
moment map and by $P = \textnormal{image\,}(\mathfrak{m})$ the moment
polytope. The symplectic manifold $(M, \omega)$ admits a canonical
$\omega$-compatible (integrable) complex structure $J_0$ which turns
$(M,J_0)$ into a complex algebraic manifold. We will refer to $J_0$ as
the {\em standard complex structure}.

Denote by $F_1, \ldots, F_r$ the codimension-$1$ facets of $P$ and by
$\overrightarrow{v_1}, \ldots, \overrightarrow{v_r} \in \mathbb{Z}^n$
the normal integral primitive vectors to the facests $F_1, \ldots,
F_r$ respectively. Note that the number of codimension-$1$ facets is
$r = n + b_2(M)$. The fibres $\mathfrak{m}^{-1}(p)$, $p \in P$, are
Lagrangian tori. There is a (unique) special point $p_* \in P$ for
which the Lagrangian torus $L = \mathfrak{m}^{-1}(p_*)$ is monotone
(see e.g.~\cite{Cho-Oh:Floer-toric, Cho:non-unitary, FO3:toric-1}).
Furthermore, we have $N_L = 2$. Note also that $H_2^D \cong
\pi_2(M,L)$, and that $r = \textnormal{rank}\, H_2^D$. We denote by
$\Sigma_i = \mathfrak{m}^{-1}(F_i) \subset M$.  These turn out to be
smooth $J_0$-complex hypersurfaces in $M$ and their sum $[\Sigma_1] +
\cdots + [\Sigma_r]$ represents the Poincar\'{e} dual of the first
Chern class $c_1$ of $M$ (which is by assumption a positive multiple
of $[\omega]$).

Since $L$ is an orbit of the $\mathbb{T}^n$-action we have a canonical
identification $H_1(L;\mathbb{Z}) = H_1(\mathbb{T}^n;\mathbb{Z})$ and
we denote by $\mathbf{e} = \{ e_1, \ldots, e_n \}$ the standard basis
corresponding to this identification.

\subsubsection{Holomorphic disks} \label{sbsb:toric-hol-disks} Due to
the $\mathbb{T}^n$-action the Lagrangian torus $L$ comes with a
prefered orientation as well as a spin structure. Fixing these two,
one can endow the space of holomorphic disks with boundary on $L$ with
a canonical orientation (see~\cite{FO3, Cho:products} for more
details).

We start with a description, due to Cho and
Oh~\cite{Cho-Oh:Floer-toric}, of the subset $\mathcal{E}_2 \subset
H_2^D$ of classes that can be represented by $J$-holomorphic disks
with Maslov index $2$ for generic $J$ (as well as for $J_0$). We use
here the notation from~\S\ref{sb:superpotential}.

\begin{prop}[Cho-Oh~\cite{Cho-Oh:Floer-toric}]
   \label{p:toric-mu=2-disks} The set $\mathcal{E}_2$ consists of
   exactly $r=\textnormal{rank}\, H_2^D$ classes $\mathcal{E}_2 = \{
   B_1, \ldots, B_r\}$ with the following properties:
   \begin{enumerate}
     \item $\# (B_i \cdot \Sigma_j) = \delta_{i,j}$ for every $i,j$.
     \item The set $\mathcal{E}_2$ is a $\mathbb{Z}$-basis for
      $H_2^D$.
     \item Denote by $\partial : H_2^D \longrightarrow
      H_1(L;\mathbb{Z})$ the boundary operator. Then writing $\partial
      B_i$ in the basis $\mathbf{e}$ we have $(\partial B_i) =
      \overrightarrow{v_i}$ for every $1 \leq i \leq r$.
     \item For every $i$, $\nu(B_i)=1$.
   \end{enumerate}
   Furthermore, the standard complex structure $J_0$ is regular for
   all classes $B \in H_2^D$ with $\mu(B)=2$. Moreover given a generic
   point $x \in L$ there exist precisely $r$ $J_0$-holomorphic disks
   $u_i: (D, \partial D) \longrightarrow (M,L)$, $i=1, \ldots, r$,
   upto paramerization, with $\mu([u_i])=2$ and $u(1)=x$. These disks
   satisfy $u_i([D])=B_i$, $i=1, \ldots, r$. The image of $u_i$ under
   the moment map $\mathfrak{m} \circ u_i$ is a straight segment going
   from the barycenter $p_*$ to a point on the facet $F_i$.
\end{prop}

\subsubsection{The superpotential, the wide variety and the
  discriminant} \label{sb:P-wide-discr-toric} The following is an
immediate corollary of Proposition~\ref{p:toric-mu=2-disks}:
\begin{cor}[Cho-Oh~\cite{Cho-Oh:Floer-toric}]
   \label{c:super-potential}
   The superpotential $\mathcal{P}$ admits
   the following form in the coordinates induced by the basis
   $\mathbf{e}$ (see~\S\ref{sbsb:sp-formulae}):
   \begin{equation} \label{eq:P-toric}
      \mathscr{P}(z_1, \ldots, z_n) = \sum_{i=1}^r 
      z^{\overrightarrow{v_i}},
   \end{equation}
   where for a vector $\overrightarrow{v}=(v^1, \ldots, v^n) \in
   \mathbb{Z}^n$, $z^{\overrightarrow{v}}$ stands for the monomial
   $z^{\overrightarrow{v}} = z_1^{v^{1}} \cdots z_n^{v^{n}}$.
\end{cor}

Since $H^1(L;\mathbb{R})$ generates $H^*(L;\mathbb{R})$ (with respect
to the cup product) we obtain from Proposition~\ref{p:dC-i}:
\begin{cor}[Cho-Oh~\cite{Cho-Oh:Floer-toric}, see also
   Fukaya-Oh-Ohta-Ono~\cite{FO3:toric-1}] \label{c:wide-crit} We have
   $$\mathcal{W}_1 = \textnormal{Crit}(\mathscr{\mathscr{P}}),$$ where
   $\mathcal{W}_1 \subset \textnormal{Hom}(H_1, \mathbb{C}^*)$ is the
   wide variety as defined in~\S\ref{s:wide}.
\end{cor}

Choose a basis $\mathbf{C} = \{C_1, \ldots, C_n \}$ for
$H_{n-1}(L;\mathbb{Z})$ which is dual to $\mathbf{e}$ as
in~\S\ref{sbsb:sp-formulae}. We view $H_{n-1}(L;\mathbb{C})$ as a
subset of $QH_{n-1}(L;\mathcal{W}_1)$ as explained
in~\S\ref{sbsb:sp-formulae} just before the statement of
Proposition~\ref{p:prod-Ci-Cj}. The following corollary immediately
follows from Proposition~\ref{p:prod-Ci-Cj}.
\begin{cor}[Cho~\cite{Cho:products}] \label{c:prod} $$C_i * C_j + C_j
   * C_i = \Bigl(\sum_{k=1}^r v_k^{i} v_k^{j} \,
   z^{\overrightarrow{v_k}} \Bigr)[L] t, \; \forall z \in
   \mathcal{W}_1.$$
\end{cor}

We now turn to the quadratic form defined in~\S\ref{s:qforms} and its
discriminant. Substituting~\eqref{eq:P-toric} in~\eqref{eq:discr-2} we
get:
\begin{equation} \label{eq:discr-toric-1} \Delta(z_1, \ldots, z_n) =
   -\det \Bigl( \sum_{k=1}^r v_k^i v_k^j \,z^{\overrightarrow{v_k}}
   \Bigr)_{i,j}, \; \forall z \in \mathcal{W}_1.
\end{equation}
However, there is a nicer formula for the discriminant which we now
present. For a subset of indices $I \subset \{1, \ldots, r\}$ with
$\#I=n$, say $I = \{i_1, \ldots, i_n\}$, define an $n \times
n$\,-matrix $A_I$ whose rows consists of the vectors
$\overrightarrow{v_{i_1}}, \ldots, \overrightarrow{v_{i_n}}$, and a
vector $\overrightarrow{v_I}$ which is the sum of the
$\overrightarrow{v_{i_k}}$'s, i.e. 
\begin{equation} \label{eq:A_I}
   A_I = 
   \begin{pmatrix}
      \textnormal{-----------} & \overrightarrow{v_{i_1}} &
      \textnormal{-----------} \\
      & \vdots & \\
      \textnormal{-----------} & \overrightarrow{v_{i_k}} &
      \textnormal{-----------} \\
      & \vdots &  \\
      \textnormal{-----------} & \overrightarrow{v_{i_n}} &
      \textnormal{-----------}
   \end{pmatrix}
   , \qquad \overrightarrow{v_I} = \sum_{i \in I} \overrightarrow{v_i}.
\end{equation}
Note that $\det(A_I)^2$ does not depend on the ordering of the indices
$i_j$ in the set $I$.

\begin{prop}
   The discriminant admist the following formula:
   \begin{equation} \label{eq:discr-toric-2} \Delta(z_1, \ldots, z_n)
      = - \sum_{\substack{I \subset \{1, \ldots, r\} \\ \#I=n}}
      z^{\overrightarrow{v_I}} \det(A_I)^2, \; \forall z \in
      \mathcal{W}_1.
   \end{equation}
\end{prop}
The proof follows by direct computation by expanding the determinant
in~\eqref{eq:discr-toric-1}. \INS some details of the proof/calculation.

\subsection{Wide varieties and quantum homology of the ambient
  manifold} \label{sb:wide-qh} Here we further study the other quantum
strucutres, such as the quantum algebra and quantum inclusion, and
their relations to the wide varieties on toric manifolds.

Let $L = \mathfrak{m}^{-1}(p_*) \subset M$ be the monotone torus fibre
in a monotone toric manifold. Assume that the wide variety
$\mathcal{W}_1$ is not empty. By Corollary~\ref{c:wide-crit} the wide
variety $\mathcal{W}_1$ coincides with the variety of critical points
of the superpotential function $\mathscr{P}$, $\mathcal{W}_1 =
\textnormal{Crit}(\mathscr{P})$, hence the ring or global algebraic
functions $\mathcal{O}(\mathcal{W}_1)$ can be written as
\begin{equation} \label{eq:O-W_1} \mathcal{O}(\mathcal{W}_1) =
   \frac{\mathbb{C}[z_1^{\pm 1}, \ldots, z_n^{\pm 1}]}{\langle
     \partial_{z_1} \mathscr{P}, \ldots, \partial_{z_n} \mathscr{P} 
     \rangle},
\end{equation}
where the denominator stand for the ideal generated by the partial
derivatives of $\mathscr{P}$. This ring, or rather localizations of
it, plays an important role in singularity theory and is sometime
called the Jacobian ring of $\mathscr{P}$.

Interestingly, this ring appears in the symplectic picture also from a
different angle. Denote by $QH(M;\Lambda)$ the quantum homology of the
{\em ambient} manifold with coeficients in $\Lambda = \mathbb{C}[t,
t^{-1}]$, where for compatability with the Lagrangian picture we put
$|t| = -N_L$. It is well known that the classes $[\Sigma_i] =
\frak{m}^{-1}(F_i) \in QH_{2n-2}(M;\Lambda)$, $i=1, \ldots, r$,
generate $QH(M; \Lambda)$ with respect to the quantum product $*$,
see~\cite{Batyrev:qh-toric, McD-Sa:Jhol-2}. It turns out that
$QH(M;\Lambda)$ is isomorphic as a ring to $\mathcal{O}(\mathcal{W}_1)
\otimes \Lambda$. More precisely:
\begin{thm}[Batyrev, Givental, Fukaya-Oh-Ohta-Ono] \label{t:Bat-Giv}
   There exists an isomorphism of rings
   \begin{equation} \label{eq:iso-I} I: QH(M; \Lambda) \longrightarrow
      \mathcal{O}(\mathcal{W}_1) \otimes \Lambda,
   \end{equation}
   which satisfies $I([\Sigma_i]) = z^{\overrightarrow{v_i}}t$. This
   isomorphism shifts degrees by $-2n$. Here, the grading on the
   right-hand side comes from the $\Lambda$-factor only (i.e.
   $\mathcal{O}(\mathcal{W}_1)$ is not graded).
\end{thm}
This theorem was first suggested by Givental~\cite{Gi:hom-geom-ICM}
and by Batyrev~\cite{Batyrev:qh-toric} and has been verified since
them at different level of rigor. A rather rigorous and conceptual
proof has been recently carried out by
Fukaya-Oh-Ohta-Ono~\cite{FO3:toric-1}. See also~\cite{Os-Ty:qh} for a
more algebraically oriented proof. It is important to note that the
isomorphism~\eqref{eq:iso-I} does not send $QH(M;\Lambda^+)$ onto
$\mathcal{O}(\mathcal{W}_1) \otimes \Lambda^+$ but rather into a
subset of the latter.

We now consider the quantum module structure on $QH(L)$.  Recall
from~\ref{sb:qh} that for a $\widetilde{\Lambda}^+$-algebrea
$\mathcal{R}$, $QH(L;\mathcal{R})$ is a module (in fact an algebra)
over $QH(M; \mathcal{R})$. We will use here $\mathcal{R} =
\mathcal{O}(\mathcal{W}_1) \otimes \Lambda$, but a similar discussion
holds for $\mathcal{O}(\mathcal{W}_1) \otimes \Lambda^+$ too. For $a
\in QH_j(M; \mathcal{O}(\mathcal{W}_1) \otimes \Lambda)$ and $\alpha
\in QH_k(L; \mathcal{W}_1)$ (see the notation in~\eqref{eq:qh-w}) we
denote by $a*\alpha \in QH_{j+k-2n}(L;\mathcal{W}_1)$ the quantum
module action.  Using the embedding $\Lambda = 1 \otimes \Lambda
\subset \mathcal{O}(\mathcal{W}_1) \otimes \Lambda$, we have a natural
inclusion $QH(M;\Lambda) \subset QH(M; \mathcal{O}(\mathcal{W}_1)
\otimes \Lambda)$. We will now take a closer look at the induced
module operation
\begin{equation} \label{eq:q-mod-W} QH(M; \Lambda) \otimes_{\Lambda}
   QH(L; \mathcal{W}_1) \longrightarrow QH(L;\mathcal{W}_1), \quad a
   \otimes \alpha \longmapsto a*\alpha.
\end{equation}
Note that $QH(L;\mathcal{W}_1)$ is also a module over
$\mathcal{O}(\mathcal{W}_1) \otimes \Lambda$ in an obvious way. For $c
\in \mathcal{O}(\mathcal{W}_1) \otimes \Lambda$, $\alpha \in
QH(L;\mathcal{W}_1)$ we denote this module operation as $c\alpha$. It
turns out that this module structure and the preceding ones are in
fact compatible:
\begin{prop} \label{p:a*alpha}
   For every $a \in QH(M; \Lambda)$ and $\alpha \in QH(L;
   \mathcal{W}_1)$ we have:
   \begin{equation} \label{eq:qmod-identity}
      a*\alpha = I(a)\alpha.
   \end{equation}
   The same continues to hold if we replace $\Lambda$ by $\Lambda^+$
   and $QH(L;\mathcal{W}_1)$ by $Q^+H(L;\mathcal{W}_1)$.
\end{prop}
\begin{proof}
   Since $QH(M;\Lambda)$ is generated by the classes $[\Sigma_i] =
   \frak{m}^{-1}(F_i)$, $i=1, \ldots, r$, it is enough to
   check~\eqref{eq:qmod-identity} for $a = [\Sigma_i]$. Since $*$ is a
   module action, it is also enough to restrict to the case $\alpha =
   [L]$ which is the unity of $QH(L;\mathcal{W}_1)$.

   Next note that $[\Sigma_i]*[L]$ lies in the image of the natural
   map $Q^+H(L;\mathcal{W}_1) \longrightarrow QH(L;\mathcal{W}_1)$
   hence it is enough to show that~\eqref{eq:qmod-identity} holds in
   $Q^+H(L;\mathcal{W}_1)$.

   Recall from~\eqref{eq:ex-seq-qh_n-2} that we have the following
   exact sequence:
   \begin{equation} \label{eq:ex-seq-W_1-qh_n-2} 0 \longrightarrow
      \mathcal{O}(\mathcal{W}_1) [L]t \stackrel{i}{\longrightarrow}
      Q^+H_{n-2}(L;\mathcal{W}_1) \stackrel{\pi} \longrightarrow
      H_{n-2}(L;\mathbb{C}) \otimes \mathcal{O}(\mathcal{W}_1)
      \longrightarrow 0.
   \end{equation}
   Moreover, it follows from the definition of the quantum module
   action that $\pi([\Sigma_i]*[L]) = [\Sigma_i]\cdot [L]$, where
   $[\Sigma_i] \cdot [L]$ stand for the classical intersection product
   in singular homology. But $L$ is disjoint from $\Sigma_i$, hence
   $\pi([\Sigma_i]*[L])= [\Sigma_i] \cdot [L] = 0$. It follows
   from~\eqref{eq:ex-seq-W_1-qh_n-2} that $[\Sigma_i]* [L] =c[L]t$ for
   some function $c \in \mathcal{O}(\mathcal{W}_1)$.

   To determine $c$ note that if we work with coefficients in
   $\widetilde{\Lambda}^+$ we have:
   \begin{equation} \label{eq:qmod-toric-wtld} [\Sigma_i]*[L] =
      \sum_{B \in \mathcal{E}_2} \#(B \cdot \Sigma_i) \nu(B) T^B [L].
   \end{equation}
   Substituting the information from
   Proposition~\ref{p:toric-mu=2-disks}
   into~\eqref{eq:qmod-toric-wtld} we immediately obtain
   $$[\Sigma_i]*[L] = z^{\overrightarrow{v_i}} [L]t.$$ Since
   $z^{\overrightarrow{v_i}} t = I([\Sigma_i])$ this concludes the
   proof.
\end{proof}

Next we consider the quantum inclusion map. Let $f:L \longrightarrow
\mathbb{R}$ be a perfect Morse function having exactly one minimum,
$x_0 \in L$. Let $(\cdot, \cdot)$ be a Riemannian metric on $L$ and
$J$ an $\omega$-compatible almost complex structure on $M$. Put
$\mathscr{D} = (f, (\cdot, \cdot), J)$ and assume the elements of this
triple have been chosen to be generic so that the pearl complex
$\mathcal{C}(\mathscr{D};\mathcal{O}(\mathcal{W}_1)\otimes \Lambda)$
is well defined. Under these assumption $x_0 \in
\mathcal{C}(\mathscr{D};\mathcal{O}(\mathcal{W}_1)\otimes \Lambda)$ is
a cycle and we denote by $[x_0] \in QH(L;\mathcal{W}_1)$ its homology
class. Note that in general $[x_0]$ strongly depends on the choice of
$\mathscr{D}$. (See~\S 4.5 in~\cite{Bi-Co:rigidity}.) Nevertheless, it
turns out that its image under the quantum inclusion~\eqref{eq:qinc}
is well defined.
\begin{prop} \label{p:iL-x_0} Let $a_1, \ldots, a_m \in
   H_*(M;\mathbb{C})$ be elements of pure degree which consist of a
   basis for the total homology $H_*(M;\mathbb{C})$. Denote by
   $a_1^{\#}, \ldots, a_m^{\#}$ the dual basis with respect to
   intersection product.  Then:
   \begin{equation} \label{eq:iL-x_0-1} i_L([x_0]) =
      \sum_{i=1}^{m}I(a_i^{\#})a_i \; \in \; QH(M;
      \mathcal{O}(\mathcal{W}_1) \otimes \Lambda).
   \end{equation}
\end{prop}
Note that we can always take $a_1 = [\textnormal{pt}] \in
H_0(M;\mathbb{C})$ to be the class of a point and $a_m = [M] \in
H_{2n}(M;\mathbb{C})$ to be the fundamental class. We will then have
$a_1^{\#}=[M]$ and $a_m^{\#} = [\textnormal{pt}]$ and
formula~\eqref{eq:iL-x_0-1} becomes:
\begin{equation} \label{eq:iL-x_0-2} i_L([x_0]) = [\textnormal{pt}] +
   \sum_{i=2}^{m-1}I(a_i^{\#})a_i + I([\textnormal{pt}])[M].
\end{equation}

In order to prove Proposition~\ref{p:iL-x_0} we will use the
augmentation map $\epsilon_L : QH(L;\mathcal{R}) \longrightarrow
\mathcal{R}$, defined for every $\widetilde{\Lambda}^+$--algebra
$\mathcal{R}$. The precise definition and properties of this map can
be found in~\cite{Bi-Co:rigidity} (see e.g. Theorem~A in that paper).
The augmentation manp $\epsilon_L$ is induced by a map
$\widetilde{\epsilon_L} : \mathcal{C}(f, \rho, J; \mathcal{R})
\longrightarrow \mathcal{R}$ which is defined as follows.  Assume that
$f$ has a unique minimum $x_0$, then $\widetilde{\epsilon_L}(x_0) = 1$
and for every $x \in \textnormal{Crit}(f)$, $x \neq x_0$,
$\widetilde{\epsilon_L}(x_0)$. It satisfies the following identity
\begin{equation} \label{eq:aug-1} \langle \textnormal{PD}(b),
   i_L(\beta) \rangle = \epsilon_L(b * \beta), \quad \forall \; b \in
   H_*(M;\mathbb{C})\subset QH(M;\mathcal{R}), \; \beta \in
   QH(L;\mathcal{R}),
\end{equation}
where $\textnormal{PD}$ stand for Poincar\'{e} duality and $\langle
\cdot, \cdot \rangle$ for the obvious $\mathcal{R}$--linear extension
of the Kronecker pairing.

We are now ready to prove Proposition~\ref{p:iL-x_0}.
\begin{proof}[Proof of Proposition~\ref{p:iL-x_0}]
   Write $i_L([x_0]) = \sum_{i=1}^{m}\varphi_i a_i$, with $\varphi_i
   \in \mathcal{O}(\mathcal{W}_1) \otimes \Lambda$. Apply now
   formula~\eqref{eq:aug-1} with $b=a_j^{\#}$, $\beta=[x_0]$. We
   obtain $$\varphi_j = \langle \textnormal{PD}(a_j^{\#}), i_L([x_0])
   \rangle = \epsilon_L(a_j^{\#} * [x_0]) =
   \epsilon_L(I(a_j^{\#})[x_0]) = I(a_j^{\#}),$$ where the one to last
   equality follows from Proposition~\ref{p:a*alpha}.
\end{proof}

\begin{rem} \label{r:Ia} In a similar way one can prove that 
   \begin{equation} \label{eq:Ia} I(a) = \langle \textnormal{PD}(a),
      i_L([x_0])\rangle, \quad \forall \; a \in H_*(M;\mathbb{C}).
   \end{equation}
\end{rem}

\subsection{The Frobenius structure and the quantum Euler class}
\label{sb:frob} The quantum homology $QH(M;\Lambda)$ has the structure
of a Frobenius algebra. In this section we show how to translate this
structure via the isomorphism $I$ to the Jacobian ring
$\mathcal{O}(\mathcal{W}_1) \otimes \Lambda$.

\subsubsection{Generalities on Frobenius algebras}
\label{sbsb:frob-gnrl} We first recall some basic notions about
Frobenius algebras. The reader is referred
to~\cite{Abrams:semi-simple} and the references therein for the
general theory of Frobenius algebras.

Let $\mathcal{A}$ be an algebra over a ring $\mathcal{R}$ and assume
that $\mathcal{A}$ is a free finite-rank module over $\mathcal{R}$. A
Frobenius structure on $\mathcal{A}$ is an $\mathcal{R}$--linear map
$F:\mathcal{A} \longrightarrow \mathcal{R}$ such that the associated
bilinear pairing
$$\mathcal{A} \otimes_{\mathcal{R}} \mathcal{A} \longrightarrow
\mathcal{R}, \quad a\otimes b \longmapsto F(ab)$$ is
non-singular in the sense that the induced map $\mathcal{A}
\longrightarrow \textnormal{Hom}_{\mathcal{R}}(\mathcal{A},
\mathcal{R})$, $a \longmapsto F(a \cdot -)$, is invertible (or put in
different terms, the associated matrix of the pairing is invertible in
some basis of $\mathcal{A}$ over $\mathcal{R}$). Of course, the
associated bilinear pairing of a Frobenius structures can be viewed as
a generalization of the notion of Poincar\'{e} duality.  Note that
when the ring $\mathcal{R}$ is not a field some authors (e.g.
Abrams~\cite{Abrams:semi-simple}) use the notion Frobenius extension
rather than Frobenius structure.

To a Frobenius structure one can associate an invariant called the
Euler class, introduced by Abrams~\cite{Abrams:semi-simple}. This is
defined as follows. Pick a basis $a_1, \ldots, a_m$ of $\mathcal{A}$
over $\mathcal{R}$. Let $a_1\spcheck, \ldots, a_m\spcheck$ be the dual
basis with respect to the Frobenius pairing. The Euler class
$\mathscr{E}(\mathcal{A}, F)$ is defined as:
\begin{equation} \label{eq:euler-A} \mathscr{E}(\mathcal{A}, F) =
   \sum_{i=1}^m a_i a_i\spcheck.
\end{equation}
It is straighforward to check that $\mathscr{E}(\mathcal{A}, F)$ does
not depend on the choice of the basis. The importance of the Euler
class comes form the following theorem.
\begin{thm}[Abrams~\cite{Abrams:semi-simple, Abrams:thesis}] 
\label{t:Abrams} Let
   $\mathcal{A}$ be a finite dimensional algebra over a field
   $\mathcal{R}$ of characteristic $0$. Then:
   \begin{enumerate}
     \item For every two Frobenius structures $F'$ and $F''$ on
      $\mathcal{A}$ there exists an invertible element $u \in
      \mathcal{A}$ such that $F'' = u F'$. Moreover we have:
      $\mathscr{E}(\mathcal{A}, F'') = u^{-1} \mathscr{E}(\mathcal{A},
      F'')$. Thus the Euler class does not depend on the Frobenius
      structure upto multiplication by an invertible element. In
      particular, whether or not the Euler class is a zero divisor, or
      whether or not it is invertible, does not depend on the
      particular choice of the Frobenius structure.
     \item Suppose that the Euler class of some (hence for every)
      Frobenius structure on $\mathcal{A}$) is not a zero divisor.
      Then the Euler class determines the Frobenius structure on
      $\mathcal{A}$ in the sense that there exists a unique Frobenius
      structure $F$ on $\mathcal{A}$ with a given Euler class.
     \item The algebra $\mathcal{A}$ is semi-simple iff the Euler
      class $\mathscr{E}(\mathcal{A}, F)$ is invertible for some
      Frobenius structures $F$ on $\mathcal{A}$.
   \end{enumerate}
\end{thm}

We also have the following result that will be relevant for our purposes.
\begin{thm}[Scheja-Storch~\cite{Sch-St:spur}] \label{t:scheja-storch}
   Let $(\mathcal{A}, F)$ be a Frobenius algebra over a field
   $\mathcal{R}$ of characteristic $0$. Suppose that $\mathcal{A}$ can
   be written as $\mathcal{A} = \mathcal{R}[x_1, \ldots, x_r]/
   \mathcal{I}$ for some ideal $\mathcal{I}$ which is generated by $r$
   elements $f_1, \ldots, f_r \in \mathcal{R}[x_1, \ldots, x_r]$. Put
   $$J = \det \Bigl(\frac{\partial f_i}{\partial x_j}\Bigr)_{i,j} \in
   \mathcal{A}.$$ If $J \neq 0$ then $J = u \mathscr{E}(\mathcal{A},
   F)$ for some invertible element $u \in \mathcal{A}$.
\end{thm}

\subsubsection{The main examples} \label{sbsb:frob-exp} Here are two
examples that are relevant in our context. The first on is classical.
Let $M$ be a closed manifold and $\mathcal{R}$ any ring.  Assume for
simplicity that $H_i(M;\mathcal{R})=0$ for every odd $i$.  Let
$\mathcal{A} = H_*(M;\mathcal{R})$ endowed with the the intersection
product $\cdot$. Write $$H_*(M;\mathcal{R}) = \mathcal{R}
[\textnormal{pt}] \; \bigoplus \bigoplus_{j=1}^{\dim M/2}
H_{2j}(M;\mathcal{R}),$$ where $[\textnormal{pt}]$ is the class of a
point. The Frobenius structure $F$ is define by the projection onto
the $\mathcal{R} [\textnormal{pt}]$ factor. In other words, $F(a)$ is
defined to be the coefficient of $a$ at $[\textnormal{pt}]$. The
associated bilinear pairing is precisely the intersection pairing. A
simple computation shows that the Eular class $\mathscr{E} =
\mathscr{E}(\mathcal{A}, F)$ in this case is exactly
$\chi(M)[\textnormal{pt}]$.

The second example, which is the one we will focus on, is the quantum
cohomology of a symplectic manifold $M$. We assume that $(M, \omega)$
is a closed monotone symplectic manifold and that
$H_i(M;\mathbb{C})=0$ for every even odd $i$. Put
$\mathcal{A}=QH(M;\Lambda)$ endowed with the quantum product $*$ and
let $\mathcal{R} = \Lambda$. The Frobenius structure is taken as in
the preceding example, i.e. for $a \in QH(M;\Lambda)$ we set $F(a)\in
\Lambda$ to be the coefficient of $a$ at $[\textnormal{pt}]$. We
denote it from now on by $F_Q$ to emphasize the realtion to quantum
homology. The fact that this is indeed a Frobenius structure is not
immediate.  It is proved e.g. in~\cite{Abrams:semi-simple}.

We now turn to the Euler class of the Frobenius structure $F_Q$ on the
quantum homology. We denote it for simplicity by $\mathscr{E}_{Q}$ and
call it the {\em quantum Euler class}. Under the assumptions that $(M,
\omega)$ is monotone and $H_{\textnormal{odd}}(M;\mathbb{C})=0$ we
have the following:
\begin{lem} \label{l:dual-basis} Let $\mathbf{a}= \{a_1, \ldots,
   a_m\}$ be a basis for $H_*(M;\mathbb{C})$ consisting of elements of
   pure degree and $\mathbf{a}^{\#} = \{a_1^{\#}, \ldots, a_m^{\#}\}
   \in H_*(M;\mathbb{C})$ be the dual basis with respect to the {\em
     classical} intersection product. Then $\mathbf{a}^{\#}$ is also a
   dual basis with respect to the quantum product $*$. In particular
   we have
   \begin{equation} \label{eq:EQ}
      \mathscr{E}_Q = \sum_{i=1}^m a_i*a_i^{\#}.
   \end{equation}
   This calss belongs to $QH_0(M;\Lambda)$ and is a deformation of the
   classical Euler class, i.e. $\mathscr{E}_Q =
   \chi(M)[\textnormal{pt}] + h.o.(t)$, where $h.o.(t)$ stands for
   higher order terms in $t$.
\end{lem}
The proof can be found in~\cite{Bi-Co:qrel-long} (see
Proposition~6.5.7 and the proof of Proposition~6.5.8 in that paper).

Note that $\Lambda$ is not a field hence Theorems~\ref{t:Abrams}
and~\ref{t:scheja-storch} do not apply for $QH(M;\Lambda)$. To go
about this difficulty we can work with the completion
$\widehat{\Lambda} = \mathbb{C}[t^{-1},t]]$ consisting of formal
Laurent series in $t$ with finitely many terms having negative powers
of $t$. Note that $\widehat{\Lambda}$ is a field. We can define in a
straightforward way $QH(M;\widehat{\Lambda})$, endowed with the
quantum product and we have an inclusion of rings $QH(M;\Lambda)
\subset QH(M; \widehat{\Lambda})$. Obviously the preceding Frobenius
structure $F_Q$ extends to $QH(M;\widehat{\Lambda})$ and the quantum
Euler class remains exactly the same. 

\subsubsection{Back to toric manifolds} \label{sbsb:back-to-toric}
We now return to the case of toric manifolds.

Suppose that the superpotential $\mathscr{P}:(\mathbb{C}^*)^{\times n}
\longrightarrow \mathbb{C}$ is a Morse function (in the holomorphic
sense), i.e. it has only isolated critical points and at each such
point the holomorphic Hessian is non-degenerate.

In this case $\mathcal{W}_1$ is a scheme consisting of a finite number
of points each coming with multiplicity $1$. Therefore
$\mathcal{O}(\mathcal{W}_1) = \bigoplus_{z \in \mathcal{W}_1}
{\mathbb{C}}$, hence by the isomorphism~\eqref{eq:iso-I} from
Theorem~\ref{t:Bat-Giv} it follows that the quantum cohomology
$QH(M;\Lambda)$ splits as: $$QH(M;\Lambda) \cong \bigoplus_{z \in
  \mathcal{W}_1} \Lambda,$$ and similarly for
$QH(M;\widehat{\Lambda})$. It follows that $QH(M;\widehat{\Lambda})$
is semi-simple. It turns out that the converse direction is also true,
hence $QH(M;\widehat{\Lambda})$ is semi-simple iff $\mathscr{P}$ is
Morse (see~\cite{Os-Ty:qh} for the proof and for more on
semi-simplicity of $QH$ for toric manifolds).

The next theorem is concerned with how the quantum Frobenius structure
and Euler class look like when they are translated to
$\mathcal{O}(\mathcal{W}_1)$ via the isomorphism~\eqref{eq:iso-I} from
Theorem~\ref{t:Bat-Giv}.

\begin{thm} \label{t:qh-frob-struct}
   Suppose that $\mathscr{P}$ is Morse. Then:
   \begin{enumerate}
     \item $I(\mathscr{E}_Q) = -\Delta t^n$, where $\Delta \in
      \mathcal{O}(\mathcal{W}_1)$ is the discriminant introduced
      in~\eqref{eq:discr-2} of~\S\ref{sb:discr}.
     \item Via the isomorphism $I$, the quantum Frobenius structure on
      $\mathcal{O}(\mathcal{W}_1) \otimes \Lambda$ has the form:
      \begin{equation} \label{eq:q-frob} F_Q(\sigma) = -\frac{1}{t^n}
         \sum_{z \in \mathcal{W}_1} \frac{\sigma(z)}{\Delta(z)}, \quad
         \forall \; \sigma \in \mathcal{O}(\mathcal{W}_1) \otimes
         \Lambda.
      \end{equation}
   \end{enumerate}
\end{thm}
We have recently learned from~\cite{FO3:toric-2} that a similar result
has been independently obtained also by Fukaya-Oh-Ohta-Ono and will be
published in a forthcoming paper. We will give only an outline of the
proof of Theorem~\ref{t:qh-frob-struct} in~\S\ref{sb:proof-qh-frob}.
Full details will appear elsewhere.

Denote by $F_1, \ldots, F_r$ the codimension-$1$ facets of the moment
polytope $P = \textnormal{image\,}(\mathfrak{m})$ and by
$\overrightarrow{v_1}, \ldots, \overrightarrow{v}_r$ the normal
integral primitive vectors to these facets as
in~\S\ref{sb:toric-setting}. For a subset of indices $I \subset \{1,
\ldots, r\}$ write $\overrightarrow{v_I} = \sum_{i \in I}
\overrightarrow{v_i}$. The following is an immediate consequence of
Theorem~\ref{t:qh-frob-struct}.
\begin{cor} \label{c:frob-sums} Assume that $\mathscr{P}$ is Morse.
   Let $I \subset \{1, \ldots, r\}$ be a subset of indices.  
   If \, $\# I < n$ then:
   \begin{equation} \label{eq:frob-sums-1} \sum_{z \in \mathcal{W}_1}
      \frac{z^{\overrightarrow{v_I}}}{\Delta(z)} = 0.
   \end{equation}
   If \, $\#I = n$ then:
   \begin{equation} \label{eq:frob-sums-2}
      \sum_{z \in \mathcal{W}_1}
      \frac{z^{\overrightarrow{v_I}}}{\Delta(z)} =
      \begin{cases}
         0, & \textnormal{if } \; \cap_{i \in I} F_i = \emptyset, \\
         -1,&  \textnormal{if } \; \cap_{i \in I} F_i \neq \emptyset.
      \end{cases}
   \end{equation}
   


\end{cor}

